Leveraging Contextual Counterfactuals Toward Belief Calibration

Beliefs and values are increasingly being incorporated into our AI systems through alignment processes, such as carefully curating data collection principles or regularizing the loss function used for training. However, the meta-alignment problem is that these human beliefs are diverse and not aligned across populations; furthermore, the implicit strength of each belief may not be well calibrated even among humans, especially when trying to generalize across contexts. Specifically, in high regret situations, we observe that contextual counterfactuals and recourse costs are particularly important in updating a decision maker's beliefs and the strengths to which such beliefs are held. Therefore, we argue that including counterfactuals is key to an accurate calibration of beliefs during alignment. To do this, we first segment belief diversity into two categories: subjectivity (across individuals within a population) and epistemic uncertainty (within an individual across different contexts). By leveraging our notion of epistemic uncertainty, we introduce `the belief calibration cycle' framework to more holistically calibrate this diversity of beliefs with context-driven counterfactual reasoning by using a multi-objective optimization. We empirically apply our framework for finding a Pareto frontier of clustered optimal belief strengths that generalize across different contexts, demonstrating its efficacy on a toy dataset for credit decisions.

==> workspace.tex <==

\section{OUTLINE}
New abstract for counterfactual workshop at ICML

MOTIVATION: 
\begin{enumerate}
    \item Values and beliefs are implicitly baked into all of our machine learning systems but how much do we understand our own values and introduce epistemic humility as a concept.
    \item However, mathematical translation of values into practical metrics can be diverse, but this leads to diverse frameworks that are impossible to reconcile due to diverse beliefs (e.g. fairness impossibility).
    \item To try to come up with a general value framework, some have come up with constitutional/principles language, for anthropic, open AI, MILA
    \item There is diversity in individuals and even in an individual, we hold beliefs to different levels of strength and there is a constant flux in due to epistemic uncertainty -> introduces Bayesian.    
    \item Even more complicated, our beliefs can be context dependent: bias in one context is not in another, even in the same belief.  (cite judging facts/judging norms and help vs harm). introduces context = different explanations or adding recourses. Also talk about legal benefit of the doubt
\end{enumerate}

CONTRIBUTIONS:
Ok so I was looking at https://arxiv.org/abs/2010.10596 and I think that we can say this:

\paragraph{What happens when beliefs lead to conflicting outcomes?} Should we be more explicit in our beliefs? Should we summarize the conflicting beliefs into one? What happens if the recourses are similar, then how much does it matter if the predicted outcomes are varied? 


Counterfactuals is about for a fixed parameters w and input x, how to find a such that f(w, x + a) has a desired change in outcome. However, our beliefs/priors affect the choice of w.

Therefore, it might be also interesting to ask: How much would the beliefs need to change such that f(w + d, x) has a desired change in outcome (if possible). This relieves the burden of "change" from solely the user and shares the burden to the provider. For example, if I didn't get into Princeton, sure it might be actionable to get a higher GPA but perhaps the real cause is affirmative action, which is not a "feature" I can change but it is an institutional choice. In some ways, this is counterfactual beliefs...demonstrating how the beliefs are different via specific examples in the x space.

 Even when beliefs/outcomes are different, if the recourses are similar, perhaps this is a way in which we can help the larger community through policy changes (by assisting in the recourse, e.g. covid prompted the US gov't to send stimulus checks) or belief changes (change the decision boundary such that it's easier to get from one outcome to another)

\paragraph{Bayesian Implementation} 
How do we mathematically model the diversity of beliefs leading to different w? We could model this using a GP, which often tunes hparams such as length scales (how important a parameter is) or noise. This gives us a distribution of outcomes. More importantly, this induces a distribution over recourses [this is novel] and perhaps we could analyze this to understand how similar or different beliefs are?

Perhaps we can measure prior overconfidence and try to induce some epistemic humility if there are enough datapoints that surprise our model? 

TLDR the thesis i'm thinking is:  model bias is best explained contrastively via counterfactuals in the parameter/w space by considering counterfactuals in both outcomes AND recourses [i.e. model A and model B might have the same outcome but drastically different recourse] and lastly good explanations need to have good coverage over diversity of parameters/beliefs so we explore how to enhance epistemic humility in our models.

\paragraph{Experiments}
Bayesian linear regression on credit card dataset. trains a linear classifier. produces a flipset for an individual

Experimentation:

find a common recourse 

try different regularizations on weighted l2 norm of the coefficients (this is a Bayesian "prior"), for ex., gender should have near-zero coefficient and other more immutable things like married or age.

For changes in regularzation, we can calculate: how does the common recourse changes, how much conflicting outcomes, and epistemic humility in terms how surprised the model is. Find variables where the resutls are senstive to the prior strength. 
How does this sensitivity change as the number of training data increases/decreases?


Problem with loose beliefs is it would induce overfitting to training data -> not enough inductive bias.

Optional: We could do a fairness/calibration study? where finding the right 

Optional: What explanation could the algorithm provide to the human along with the distribution and outcomes to help guide them toward a "better belief"? (Note that human in the loop can mean both having the human create an idealized dataset to the best of their ability, but also recognizing when the previous ``idealized dataset'' falls short, perhaps in a new context. 

Feedback loop: 
create a feedback loop between belief, policy, outcome/recourse, back to belief
link to slides: 
\href{https://docs.google.com/presentation/d/1KfrQCvPFcT90m-NaVCy_dY8d3KnUReNdiQsNH4AoJ7A/edit?usp=sharing}{slides with diagram}


Old Sectional Outline:

\begin{enumerate}
    \item Intro
    \item Preliminaries / Related Work
    \item Diversity of beliefs (formalized through Bayesian reasoning [outcomes -> beliefs]) [sherol (real-life examples?)/richard (technical)]
    \item Contextual Counterfactuals (with Beliefs and Recourse and Why Diversity is Crucial [policy -> outcomes] ) [mike]
    \item Calibrative Alignment and Experiments [beliefs -> policy] (richard)
\end{enumerate}

New Sectional Outline:

\begin{enumerate}
    \item Intro
    \item Related Work (counterfactuals, [Bayesian] multi-task learning)
    \item Context Drives Diversity and Uncertainty in Beliefs
    \item heree
    \item Modeling Diversity of Beliefs
    \item Calibration and Alignment Experiments (credit card dataset
    \begin{enumerate}
        \item selection of strengths that minimizes cost of recourse and log probability (model selection)
        \item exploration of recourse on 
    \end{enumerate}
\end{enumerate}





\todo{We need a way of summarizing the distribution of outcomes and recourses back to the human. Maybe something like ``Examples are not Enough, Learn to Criticize! Criticism for Interpretability'' to select prototypical outcomes/recourses along with outliers?}

\todo{Note: all text below is from the previous Active Fairness work that can be incorporated as needed into the document above}

\subsection{Counterfactual Explanations}

Explanations that make value alignment transparent to the public is essential to taking a more nuanced approach to bias awareness in the general public. Efforts like model cards \citep{mitchell2019model} already try to provide transparency into the model mechanisms, as well as its benchmarked performance. Active fairness supplements these efforts by adding bias visibility and incorporating fairness metrics, as well as any remediation and adjustment metrics, for the multiple parties involved. More importantly, as fairness is an inherent multi-objective optimization, greater visibility in understanding the full trade-off curve, or Pareto frontier, will help users grasp the complexity behind these ML decisions.

\begin{quote}
Researchers and practitioners ought to be intentional and explicit about worldviews and value assumptions—the systems they design will always encode some belief about the world. \citep{friedler2021possibility}
\end{quote}

\subsection{Our Contributions}

In this paper, we introduce an active framework for understanding, illuminating, and even embracing for bias in our machine learning systems by examining the diverse representation of beliefs about bias and fairness \citep{andrus2021we}.
Instead of trying to detect and fully eliminate different expressions of beliefs and values, we recommend systemically introducing {\it positive} sources of bias to correct for inevitable errors. Furthermore, we posit that the simple act of explanations of different beliefs can serve to largely mitigate the harmful societal effect of reinforcing one worldview. We emphasize these core principles are grounded in fundamental religious principles, such as the Jewish belief that all life are cherished equally due to its inherent value as beloved images of the one deity or the Christian belief that grace and forgiveness are at the center of its justice and fairness systems.

\subsection{ML Fairness Intro} (Can be relegated to related work)

In ML fairness, there has been identified a variety of the negative externalities that an unchecked development of AI can produce, from historical and representation bias to algorithms that exploit human tendencies \citep{suresh2021framework}. Far worse is the reinforcing feedback loop that such biases can cause. With human values and biases baked into the datasets, annotations, model and algorithms that we run, user interaction with these algorithms can produce unintended shifts in our set of beliefs and worldviews, which ultimately dictate our actions, leading to greater biases in more recent data \citep{lerman2014leveraging}. 

In light of this, there has been a general push for a bias busting approach to slowly eliminate any perpetuation of existing bias, which are often indirect. For example, software used by courts in the United States to make pretrial detention and release decisions, known as COMPAS, measures the recidivism risk of a person. Even though the model did not specifically include race into its features, a famous investigation into the software found a bias against African-Americans, showing that it is more likely to have higher false positive rates for African-American offenders than for
Caucasian offenders \citep{mehrabi2021survey}. More subtle is the use of residential zip code as a feature in learning algorithms for important decisions such as loan applications. Even though the use of zip code appears to be innocuous and non-sensitive, it is likely to correlate with race because of the population of residential areas and is flagged as a form of technological redlining \citep{rice1996race}.

Legal and judicial biases in the United States usually favor the defendant, such as the famous adage of "innocent until proven guilty" \cite{baradaran2011restoring}. The presumption of innocence is only one of many judicial laws in the America that protect the rights of the defendant from negative legal ramifications. These principles are based on the religious and constitutional principles that founded America. At the heart of these laws is the idea of giving people with little recourse the "benefit of the doubt". 

Incorporating uncertainty into predictive distributions is at the heart of Bayesian methods in ML \cite{theodoridis2015machine}. Uncertainty can be divided in two types which are epistemic and aleatory uncertainty \citep{der2009aleatory}. Aleatory uncertainty, from the Latin word meaning “the roll of the dice”, captures the most natural notion of uncertainty that is inherent in the random outcome of a phenomena. Epistemic uncertainty encapsulates second-order uncertainty derived from knowledge-based gaps in the understanding of a parameter or process. Specifically, aleatory uncertainty states that tossing a coin will have two possible outcomes, while epistemic uncertainty questions whether the coin is fair and will give a equal chance of heads or tails.

